Analysis of HAT-P-16b and TrES-3b Exoplanets by the Transit Timing Variations Method

In this study, the transit observations of HAT-P-16b and TrES-3b exoplanets were carried out at \c{C}\"U UZAYMER Observatory with a 50 cm Ritchey Chretien type telescope. By analyzing the light curves of both exoplanets, system parameters have been obtained with acceptable models. Some of these parameters for HAT-P-16 systems were found to be: M$_{P}$=4.172$\pm$0.163 M$_{J}$, R$_{P}$=1.309$\pm$0.111 R$_{J}$, a/R$_{*}$=7.1922$\pm$0.0017 and b=0.1003$\pm$0.1533 which are consistent with the values given in \cite{2010ApJ...720.1118B}. Also, for the TrES-3 system, the same parameters were calculated as M$_{P}$=1.959$\pm$0.111 M$_{J}$, R$_{P}$=1.320$\pm$0.169 R$_{J}$, a/R$_{*}$=6.0656$\pm$ 0.4899 and b=0.7892$\pm$0.0700. These values are also consistent with the values given in \cite{2007ApJ...663L..37O}. No significant Transit Timing Variations (TTV) was found as a result of the Lomb-Scargle (LS) periodogram for HAT-P-16b by using the transit times obtained from the transit light curves (False Alarm Probabilities -- FAP) = \%96). However, a significant periodicity was found at 32.38 days and a secondary periodicity was found at 41.07 days were determined as a result of the LS periodogram obtained from the TrES-3b data. We interpret that these periods with FAP of 3.41 \% and 1.88 \%, respectively, are close to the rotation period of the host star. Therefore, these periods could be due to the modulation of spot-induced light variations.

==> review.tex <==
1.HAKEM:
-Giriş kısmında bazı kelimeler düzeltilmelidir. örneğin: "yörüge" > yörünge.
%YAPILDI, Bunun dışında yazım hatalı bulundu ve düzeltildi.
-Giriş kısmında ETD 'ye referans verilmeli.
%YAPILDI

- Okuyucu, makalede kullanılan teleskoplar (UT50, IST60, ATA50 ve T100) hakkında daha fazla bilgiye sahip olabilmesi için teleskop ve optik sistemleri hakkında daha detaylı bilgiler verilmesinde fayda var.
%YAPILDI

- AstroImageJ (AIJ) için referans verilmelidir. 
%YAPILDI

-ETD’den alınan geçiş zamanlarının hangi DQ (Data quality) değerleri aralığında alındığı metin içerisinde yazılmalıdır. Örneğin; 1-3 DQ olanlar kullanılmıştır gibi. 
%YAPILDI

-TrES-3b için TESS verilerinin ışık eğrileri verilmesi önerilir (sadece bir kaynak için neden konulduğu belirtilmedir). 
%YAPILDI (TESS IŞIK EĞRİLERİ EKLENDİ)

- Şekillerin çoğunun çözünürlüğü kötü olup bazıları hiç okunmamaktadır. Bu şekillerin daha iyi bir çözünürlükte oluşturulması gerekmektedir. Ayrıca şekillerin etiketlerinin Türkçeleştirilmesi önerilir. 
%YAPILDI

- EXOFAST v1 ile sistem parametrelerini hesaplama süreci daha detaylı anlatılabilir. 
%YAPILDI

- Bazı satırların sonlarında kelimeler yanlış kesilmiştir. örneğin "analizlerinde, hesaplanan, pro-gramında" gibi. bunların Türkçe yazım kurallarına göre düzeltilmesi önerilir.
%Bunu editor daha sonra halledecek. Bizimle ilgili geğil.



2.HAKEM:
Bu rapor, çalışmanın küçük değişiklikle yayınlanmasını uygun görür. Bu çalışma, ÇÜ UZAYMER Gözlemevi’nde bulunan 50 cm (UT50) Ritchey Chretien tipi teleskobu ile gözlenmiş HAT-P-16 b gezegeninin 4 geçiş ışık eğrisi ve TrES-3 b gezegeninin 9 geçiş ışık eğrisinin veri ve grafiğini içermekle birlikte IST60 ve T100 teleskopları gözlemleri dahil olmak üzere önceki çalışmalardan alınmış geçiş zamanı verilerini kullanmaktadır. Geçiş ışık eğrileri, EXOFAST (Eastman et al. 2013) yazılımıyla modellendikten sonra, geçiş zamanları belirlenmiştir (Aladağ 2021). Bu çalışmada HAT-P-16b ve TrES-3b’nin TTV’sindeki olası frekansların belirlenebilmesi için LS periyodogramına dayanan ve emcee paketi fonksiyonlarıyla (Foreman-Mackey et al. 2013) işleyen bir Python kodu kullanılmıştır. HAT-P-16b gezegenin kütlesi 4.172±0.163 MJ , yarıçapı 1.309±0.111 RJ ve yörüngesinin yarı-büyük eksen uzunluğu a/R_yıldız 7.1922±0.0017 ve etki parametresi b=0.1003±0.1533 bulunmuş olup 2010ApJ...720.1118B, 2013A&A...557A..30C, 2011A&A...533A.113M çalışmalarında verilen değerler ile uyumlu olduğu görülmüştür. Aynı şekilde TrES-3b gezegeninin kütlesi 1.959±0.111 MJ , yarıçapı 1.320±0.169 RJ ve yörüngesinin yarı-büyük eksen uzunluğu a/R_yıldız 6.0656±0.4899 ve etki parametresi b=0.7892±0.0700 bulunmuş olup 2012IAUS..282..135V, 2007ApJ...663L..37O, 2011PASJ...63..301L, 2017NewA...55...39P, 2020AJ....160...47M çalışmalarında sunulan değerler ile uyumludur. UT50, T100, IST60, TESS ve amatör ve profesyonel gözlemcilerin çok sayıda verisini içeren ETD veri tabanı dahil olmak üzere HAT-P-16b’nin 54 geçiş ortası zamanı, TrES-3b’nin 285 geçiş ortası zamanı toplanmış, bunlardan O-C grafikleri elde edilmiş, O-C analizlerinden elde edilen TTV grafiklerine doğrusal fit (model) uygulanmış, T0 ve P düzeltmesi yapılmıştır.
%Hakem Makakeyi tanıtıyor.

Yalnız, çizelgelerde HAT-P-16b’nin sadece UT50, ATA50 ve TESS'den alınan 12 geçiş ortası zamanı ve O-C değerlerine; TrES-3b'nin sadece UT50, T100, IST60 ve TESS'den alınan 49 geçiş ortası zamanı ve O-C değerlerine yer verilmiştir. Ayrıca modellemenin ve belirsizlik tahmininin hangi yöntemle yapıldığının (en küçük kareler, maximum likelihood, vb.) belirtilmesi faydalı olacaktır.
%YAPILDI "exofast-v1'in web tabanlı versiyonu hız açısından Nelder-Mead optimizasyon (ameoba ya da downhill simplex) algoritmasına dayalı bir stratejiyle parametre uzayında veriyle model arasında en küçük farkları verecek şekilde parametrelerin optimize değerlerini bulmaya dayanan bir yöntemle uyumlama yapmaktadır."

HAT-P-16b’nin frekans analizinde bulunan 64.63 günlük dönemin FAP değeri çok yüksek (\% 99.6) olduğundan istatistiksel olarak anlamlı olmadığı söylenmiş ve değişiminin izlenmesi gerektiği önerilmiştir. TrES-3b’nin frekans analizinde elde edilen LS periyodogramı sonucunda 32.38 günlük bir baskın dönem (FAP=\%3.41) ve 41.07 günlük ikincil dönem (FAP=\% 1.88) tespit edilmiş, güncel bir çalışma olan Mannaday et al. (2020) çalışmasında verilen 29.78 günlük değişime çok yakın olduğu; bu değişimin, yüzey sıcaklığı 5720K olan barınak yıldızda olası lekenin dönme modülasyonundan kaynaklı olduğuna işaret ettiğinin düşünüldüğü ifade edilmiş; fakat yıldızın dönme dönemi üzerine herhangi bir inceleme sunulmamıştır.
%YAPILDI (YILDIZIN DÖNME DÖNEMİ İÇİN VANCO. ET AL. 2013 ÇALIŞMASI REFERANS GÖSTERİLMİŞTİR)

Yazarın sonuç bölümünde sunduğu bulguların yapılan çalışma kapsamında anlamlı olduğu görülmektedir. Çift yıldızların dönem değişimi çalışmalarından bilindiği; 2013ApJS..208...16M, 2018A&A...615A..79V çalışmalarında da görüldüğü üzere O-C bulguları; veri kalitesi, veri sayısı ve minimum zamanı belirleme yöntemine çok bağlıdır.


* AstroImageJ (AIJ) yazılımından bahsedilmiş fakat atıf yapılmamıştır. Yapılması gereken atıf şöyledir: Collins K. ve Kielkopf J., 2013. AstroImageJ: ImageJ for Astronomy. https://ui.adsabs.harvard.edu/abs/2012APS..TSF.E9028R
%YAPILDI

==> table_old.tex <==
\begin{table}
	\centering
	\caption{HAT-P-16 sistem parametrelerinin bu çalışma ve önceki çalışmalardaki değerleri (a ve b ile gösterilen parametreler (\ref{eq1}) ve (\ref{eq2}) denklemleri ile hesaplanmıştır. Hata yerine hataların standart sapması kullanılmıştır.) Kütleçekim odaklama parametresi olarak tanımlanan Safronov sayısı (\ref{eq3}) denklemi ile hesaplanmıştır.}
	\begin{tabular}{@{}l@{~}l@{~}l@{~}l@{}}
	\hline\hline
	{Parametre} & {Birimi} & {Bu Çalışma} & {\cite{2010ApJ...720.1118B}} \\
	\hline
	$a/R_*$ & - & 7.192$\pm$0.002 & 7.17$\pm$ 0.28 \\
	Etki parametresi (b) & -& 0.102$\pm$0.153 & 0.439$\pm$0.065\\
	Delta (geçiş derinliği) & - & 0.0120$\pm$0.002 & - \\
	Yıldız yoğunluğu ($\rho$) & cgs & 0.914$\pm$0.001 & 2.42$\pm$ 0.35 \\
	Demir bolluğu [Fe/H] & dex & 0.165$\pm$0.006 & 0.17$\pm$0.08 \\
	Dış merkezlilik(e) & - & 0.027$\pm$0.079 & 0.036$\pm$0.004 \\
	Eğim (i) & Derece & 89.19$\pm$1.20 & 86.6$\pm$0.7 \\
	Periyod (P) & Gün & 2.7760 Sabit & 2.7760$\pm$3.$10^{-6}$ \\
	Yarı-büyük eksen (a)& AU & 0.0412$\pm$2.$10^{-5}$ & 0.0413$\pm$ 0.0004 \\
	Yarıçap ($R_p$) & $R_J$ & 1.31$\pm$0.11 & 1.29$\pm$0.07 \\
	Kütle ($M_p$) & $M_J$ & $4.172^a\pm0.163^b$ & 4.193$\pm$0.094 \\
	Denge sıcaklığı(Teq) &Kelvin & 1625$\pm$& 1626$\pm$\\
	Safronov sayısı ($\Theta$) & - & 0.221 & 0.220$\pm$0.011 \\
	\hline\hline
	\label{T:hatp_res}
	\end{tabular}
\end{table}

\begin{table}
	\centering
	\caption{TrES-3 sistem parametrelerinin bu çalışma ve önceki çalışmalardaki değerleri (a ve b ile gösterilen parametreler (\ref{eq1}) ve (\ref{eq2}) denklemleri ile hesaplanmıştır. Hata yerine hataların standart sapması kullanılmıştır.) Kütleçekim odaklama parametresi olarak tanımlanan Safronov sayısı (\ref{eq3}) denklemi ile hesaplanmıştır.}
	\begin{tabular}{@{}l@{~}l@{~}l@{~}l@{}}
	\hline\hline
	{Parametre} & {Birimi} & {Bu Çalışma} & {\cite{2007ApJ...663L..37O}} \\
	\hline
	$a/R_*$ & - & 6.066$\pm$0.016 & 6.06$\pm$0.10 \\
    Etki parametresi (b) & -& 0.789$\pm$0.070 & 0.828$\pm$0.010\\
    Delta (geçiş derinliği) & - & 0.0276$\pm$0.0053 & - \\
    Yıldız yoğunluğu ($\rho$) & cgs & 2.523$\pm$0.666 & - \\
    Demir bolluğu [Fe/H] & dex & -0.190$\pm$0.001 & - \\
    Dış merkezlilik(e) & - & 0.0016$\pm$0.0092 & 0\ - \\
    Eğim (i) & Derece & 82.28$\pm$1.06 & 82.15$\pm$0.21 \\
    Periyod (P) & Gün & 1.3062 Sabit & 1.3062$\pm$1.10$^{-5}$ \\
    Yarı-büyük eksen (a)& AU & 0.0223$\pm$4.10$^{-5}$ & 0.0226$\pm$ 0.0013 \\
    Yarıçap ($R_p$) & $R_J$ & 1.32$\pm$0.17 & 1.29$\pm$0.08 \\
    Kütle ($M_p$) & $M_J$ & 1.959$^a\pm0.111^b$ & 1.920$\pm$0.23 \\
    Denge sıcaklığı(Teq) & Kelvin & 1626$\pm$61 & 1643\ - \\ 
    Safronov sayısı ($\Theta$) & - & 0.073 & - \\
	\hline\hline
	\label{T:tres_res}
	\end{tabular} 	
\end{table}
